Unified Structure Generation for Universal Information Extraction

Information extraction suffers from its varying targets, heterogeneous structures, and demand-specific schemas. In this paper, we propose a unified text-to-structure generation framework, namely UIE, which can universally model different IE tasks, adaptively generate targeted structures, and collaboratively learn general IE abilities from different knowledge sources. Specifically, UIE uniformly encodes different extraction structures via a structured extraction language, adaptively generates target extractions via a schema-based prompt mechanism - structural schema instructor, and captures the common IE abilities via a large-scale pre-trained text-to-structure model. Experiments show that UIE achieved the state-of-the-art performance on 4 IE tasks, 13 datasets, and on all supervised, low-resource, and few-shot settings for a wide range of entity, relation, event and sentiment extraction tasks and their unification. These results verified the effectiveness, universality, and transferability of UIE.

==> tables/uie.tex <==
\begin{table}[t]
\centering
  \setlength{\belowcaptionskip}{-0.5cm}
\resizebox{0.44\textwidth}{!}{

\begin{tabular}{ccc}
\toprule
\textbf{Dataset} & \textbf{Domain} & \textbf{Task} \\
\midrule
ACE04 & hybird & Entity \\
ACE05-Ent & news, speech & Entity \\
CoNLL03 & news  & Entity \\
ACE05-Rel & news, speech & Entity, Relation \\
SciERC & scientific & Entity, Relation \\
CoNLL04 & news  & Entity, Relation \\
NYT   & news  & Entity, Relation \\
ACE05-Evt & news, speech & Event \\
CASIE & cybersecurity & Event \\
SemEval-14 Lap & reviews & Sentiment \\
SemEval-14 Res & reviews & Sentiment \\
SemEval-15 Res & reviews & Sentiment \\
SemEval-16 Res & reviews & Sentiment \\
\bottomrule
\end{tabular}

}

\caption{
    Universal Information Extraction Tasks.
}
\label{tab:uie}
\end{table}
